Strong coupling and quark masses from lattice QCD

I review lattice QCD calculations of the strong coupling and quark masses.

==> history.tex <==
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%



\begin{figure}
\centering
\includegraphics[%
  scale=0.4,
  angle=0,
  origin=c]{figures/ms_history.ps}
\caption{History of $m_s$ in PDG summary}
\end{figure}









